A Short-Term Predict-Then-Cluster Framework for Meal Delivery Services

Micro-delivery services offer promising solutions for on-demand city logistics, but their success relies on efficient real-time delivery operations and fleet management. On-demand meal delivery platforms seek to optimize real-time operations based on anticipatory insights into citywide demand distributions. To address these needs, this study proposes a short-term predict-then-cluster framework for on-demand meal delivery services. The framework utilizes ensemble-learning methods for point and distributional forecasting with multivariate features, including lagged-dependent inputs to capture demand dynamics. We introduce Constrained K-Means Clustering (CKMC) and Contiguity Constrained Hierarchical Clustering with Iterative Constraint Enforcement (CCHC-ICE) to generate dynamic clusters based on predicted demand and geographical proximity, tailored to user-defined operational constraints. Evaluations of European and Taiwanese case studies demonstrate that the proposed methods outperform traditional time series approaches in both accuracy and computational efficiency. Clustering results demonstrate that the incorporation of distributional predictions effectively addresses demand uncertainties, improving the quality of operational insights. Additionally, a simulation study demonstrates the practical value of short-term demand predictions for proactive strategies, such as idle fleet rebalancing, significantly enhancing delivery efficiency. By addressing demand uncertainties and operational constraints, our predict-then-cluster framework provides actionable insights for optimizing real-time operations. The approach is adaptable to other on-demand platform-based city logistics and passenger mobility services, promoting sustainable and efficient urban operations.

==> Chapters/Methodology.tex <==
\subsection{Adaptive forecasting with lagged dependent features}
\label{subset:Adaptive}
Even though a series of features can be generated based on our external knowledge or prior observation of the data, some underlying unexpected events might happen and significantly influence the target outcomes, which are not captured by the inputs. Those unexpected events can be a temporal change in opening hours of the restaurants, operational decisions made by the restaurants or the platform because the kitchen is too busy handling previous orders or the local delivery team is understaffed. These events are common in practice and typically impact the near future demand level. Nevertheless, they are difficult to be predicted and even uneasy to be spotted on the system. 
One idea to handle such problems in forecasting is by letting the forecasting model reflect the current demand level in its next prediction. In this study, we propose an adaptive forecasting mechanism with lagged dependent (LD) features, a hybrid solution to combine machine learning predictors with lagged dependent information.

Lagged dependent variables of demand data are values of demands from past periods. 
The idea of combining lagged dependent variables with machine learning regressor is inspired from conventional time series autoregressive model, and subsequence time series clustering \cite{chen2005making,aghabozorgi2015time}. 
The autoregressive model attempts to find out a linear relation between $y_t$ and its lagged dependent (LD) terms. For an autoregressive model with $p$ LD terms, $y_t$ is estimated as: $\hat{y_t} = \alpha + \sum_{i=1}^{p}\beta_i y_{t-i} + \epsilon_t$. Subsequence time series clustering is developed in the field of data mining. Instead of looking for a linear expression among observations, it detects the reoccurring patterns of time series subsequence and utilizes those recognized patterns for prediction. Typically, a sliding window is used to divide a long time series into subsequences, after which distance measurement is used to cluster those subsequences into a couple groups based on similarity \cite{aghabozorgi2015time}. Both models make use of groups of neighboring observations, which they believe to be a proxy of the current level for the dependent variable. 

Studies have been done to generate adaptive machine learning demand predictors using lagged dependent inputs. In the case of short-term electricity demand forecasting \cite{al2018short}, multivariate adaptive regression splines analysis (MARS) and support vector machines are extended with up to three half-hourly and hourly lagged inputs. Zareipour et al. \cite{zareipour2006forecasting} evaluate the performance of MARS by experimenting with a different number of lags (from 1 to 377) with a short-term energy price prediction application. 

The amount of lagged dependent features considered in our study is selected to be 4 for two practical reasons. First, we assume the adaptive information is temporary. With these lagged features, the model includes the demand information from the recent one hour.
Second, with regular hourly seasonality captured by the feature \textit{hour}, including a lag further than four 15-minute time windows may influence the seasonality effect estimated by \textit{hour}.
Recall from the literature that short-term demand forecasting with random forest regression and gradient boosting machines often achieve satisfactory outcomes in empirical studies. We choose random forest regression (RF) and eXtreme Gradient Boosting (XGBoost) as our baseline models. Note that XGBoost is the more regularized version of Gradient Boosting and, therefore, less prone to over-fitting \cite{chen2016xgboost}.

Inspired from the previous research, we propose adaptive lagged dependent random forest regression (LD-RF) and lagged dependent xgBoost (LD-XGBoost) by adding four lagged dependent features $y^{\alpha}_{i-1}$, $y^{\alpha}_{i-2}$, $y^{\alpha}_{i-3}$, $y^{\alpha}_{i-4}$ to the original set of input features for the demand prediction model of pick-up zone $\alpha$. 

\subsection{Probabilistic Forecasting by Random Forest Regression} \label{subsec:quantile}

Random forest regression (RF) has been shown by Hess \cite{hess2021real} that it is a promising machine learning predictor in the application of demand forecasting for OMDPs, as does by other applications in the history of demand forecasting. By default, a prediction provided by an RF is the mean value among all the predictions generated by each tree in the forest. 
By additionally recording samples assigned to each leaf of each tree in the forest, Meinshausen \cite{meinshausen2006quantile} designs quantile regression forests (QRF) which can generate conditional quantile predictions. QRF is essentially an ensemble of quantile decision trees where the quantile predictions given each tree are computed from the empirical distributions of observations in the leaf. 
In this section, we explain how probabilistic predictions are generated by QRF, starting with an explanation for the regular deterministic forecasting of RF. The mathematical explanations in this section follow the deductions provided by \cite{meinshausen2006quantile}. 

\subsubsection{Point forecasting of Random Forest Regression}
Let us define $Y$ as the target variable with $i = 1,2 \dots, n$ observations, and $X$ the feature vectors or predictor variable of $y$. The trained random forest regression model is denoted by $H := \{h_1,h_2,\dots,h_B\}$, where $h$ are the single tree regressor of $H$. Assume that there is a new feature vector $x$ to be predicted, we can define the prediction of a single tree $h$ by
\begin{equation} \label{eq:singletree}
    \text{single tree: \quad} \hat{\mu}(x,h) = \sum_{i=1}^{n} \omega_i(x,h) \cdot y^{*}_i ,
\end{equation}
where $y^{*}$ is the historical target values assigned to tree $h$ and $\omega_i$ is a weight function which sums to 1 for all $i$. It can be defined as 
\begin{equation} \label{eq:weight_ih}
    \omega_i(x,h) = \frac{\mathds{1}(X_i\in R_{l(x,h)})}{\#\{j: X_j \in R_{l(x,h)}\}},
\end{equation}
where $l(x,h)$ is the leaf that $x$ ends at tree regressor $h$. The indicator function equals 1 if $X_i$ shares the same leaf $l(x,h)$ with $x$, otherwise 0. The mathematical expression $\#$ is short for cardinality. And $l(x,h)$ corresponds to a rectangular subspace $R_{l(x,h)}$. 

In random forest regression, the point forecasts are produced by averaging the results from each of the $B$ trees. Hence, the average weight function of $x$ by random forest regression $H$ is denoted as,
\begin{equation} \label{eq:weight_rf}
    \omega_i(x) = \frac{1}{B} \sum_{h \in H} \omega_i(x,h).
\end{equation}
Thus, the point prediction of $x$ is given by
\begin{equation} \label{eq:point_rf}
    \text{random forest regressions:\quad} \hat{\mu}(x) = \sum_{i=1}^{n} \omega_i(x) \cdot Y_i,
\end{equation}
which is a weighted sum over all the sample $Y$ from the training data \cite{meinshausen2006quantile}.

\subsubsection{Probabilistic Forecasting from Quantile Regression Forest}
Given the set of observations $Y$ from the training data and the weight function (Equation \eqref{eq:weight_rf}) of random forest, the conditional distribution function of $Y$ can be transformed into the following, as divided in \cite{meinshausen2006quantile}:
\begin{equation} \label{eq:qrf}
    \hat{F}(y|X=x) = E(\mathds{1}(y \geq Y)) | X=x) = \sum_{i=1}^{n} \omega_i(x) \cdot \mathds{1}(y \geq Y_i),
\end{equation}
The algorithm of the complete quantile regression forest method by \cite{meinshausen2006quantile} is presented in pseudocode \ref{alg:qrf}. We should point out that the training process is mainly the same as the regular random forest regression, which outputs deterministic predictions. However, QRF records all the observations on each leaf of every tree in the forest, not merely the average. 

Likewise, we can also extend QRF into an adaptive regressor by adding lagged dependent features as suggested in Section \ref{subset:Adaptive}. The lagged-dependent quantile regression forest (LD-QRF) combines both innovations we propose in this research.

\input{PseudoCodes/Quantile Regression Forest}

==> Chapters/New_Ch03_Problem_Description.tex <==
The task of short-term demand forecasting requires the predictions to be generated for the next short time interval. It is considered more challenging than long-term predictions since the data tends to be noisy and intermittent. It means the time series can be sparse and susceptible to stochastic events, especially when the aggregated spatial and temporal \textcolor{black}{granularity} is small \cite{nikolopoulos2021we}. However, the development of fast and accurate short-term demand predictions is an unavoidable challenge for on-demand service platforms where immediate operational decisions are required to effectively respond to the ever-changing demand dynamics.
The other challenge that frequently arises in demand forecasting is complex seasonality, meaning multiple seasonal patterns may coexist.

While finer time and geographic resolutions can offer more precise operational insights to guide efficient operations of platforms, they also pose increased challenges to the forecasting models due to the noisy data. The potential for higher-resolution demand prediction remains relatively unexplored in the field, but its successful implementation could significantly enhance the efficiency and effectiveness of proactive operations and enable frequent policy updates for the platforms.
